A Better Bound Gives a Hundred Rounds: Enhanced Privacy Guarantees via $f$-Divergences

We derive the optimal differential privacy (DP) parameters of a mechanism that satisfies a given level of R\'enyi differential privacy (RDP). Our result is based on the joint range of two $f$-divergences that underlie the approximate and the R\'enyi variations of differential privacy. We apply our result to the moments accountant framework for characterizing privacy guarantees of stochastic gradient descent. When compared to the state-of-the-art, our bounds may lead to about 100 more stochastic gradient descent iterations for training deep learning models for the same privacy budget.

==> reference.tex <==
@ARTICLE{fdivergence_Sason16,
author={I. {Sason} and S. {Verd\'u}},
journal={IEEE Transactions on Information Theory},
title={$f$-Divergence Inequalities},
year={2016},
volume={62},
number={11},
pages={5973-6006},
}

@book{tuffery2011data,
  title={Data mining and statistics for decision making},
  author={Tuff{\'e}ry, St{\'e}phane},
  volume={2},
  year={2011},
  publisher={Wiley Chichester}
}

@article{polyanskiy2010channel,
  title={Channel coding rate in the finite blocklength regime},
  author={Polyanskiy, Yury and Poor, H Vincent and Verd{\'u}, Sergio},
  journal={{IEEE} Trans. Inf. Theory},
  volume={56},
  number={5},
  pages={2307--2359},
  year={2010},
  publisher={IEEE}
}

@inproceedings{makhdoumi2014information,
  title={From the information bottleneck to the privacy funnel},
  author={Makhdoumi, Ali and Salamatian, Salman and Fawaz, Nadia and M{\'e}dard, Muriel},
  booktitle={Proc. of {IEEE} Information Theory Workshop (ITW)},
  year={2014}
}

@inproceedings{hsu2018generalizing,
  title={Generalizing Bottleneck Problems},
  author={Hsu, Hsiang and Asoodeh, Shahab and Salamatian, Salman and Calmon, Flavio P},
  booktitle={Proc. of IEEE Int. Symp. Inf. Theory (ISIT)},
  year={2018}
}

@inproceedings{kairouz2014extremal,
  title={Extremal mechanisms for local differential privacy},
  author={Kairouz, Peter and Oh, Sewoong and Viswanath, Pramod},
  booktitle={Proc. of Advances in Neural Information Processing Systems (NeurIPS)},
  year={2014}
}

@inproceedings{duchi2013local,
  title={Local privacy and statistical minimax rates},
  author={Duchi, John C and Jordan, Michael I and Wainwright, Martin J},
  booktitle={Proc. of {IEEE} Foundations of Computer Science (FOCS)},
  year={2013}
}

@article{dwork2014algorithmic,
  title={The algorithmic foundations of differential privacy},
  author={Dwork, Cynthia and Roth, Aaron and others},
  journal={Foundations and Trends{\textregistered} in Theoretical Computer Science},
  volume={9},
  number={3--4},
  pages={211--407},
  year={2014},
  publisher={Now Publishers, Inc.}
}

@article{donsker1983asymptotic,
  title={Asymptotic evaluation of certain Markov process expectations for large time. IV},
  author={Donsker, Monroe D and Varadhan, SR Srinivasa},
  journal={Communications on Pure and Applied Mathematics},
  volume={36},
  number={2},
  pages={183--212},
  year={1983},
  publisher={Wiley Online Library}
}

@article{nguyen2010estimating,
  title={Estimating divergence functionals and the likelihood ratio by convex risk minimization},
  author={Nguyen, XuanLong and Wainwright, Martin J and Jordan, Michael I},
  journal={{IEEE} Trans. Inf. Theory},
  volume={56},
  number={11},
  pages={5847--5861},
  year={2010},
  publisher={IEEE}
}

@book{boyd2004convex,
  title={Convex optimization},
  author={Boyd, Stephen and Vandenberghe, Lieven},
  year={2004},
  publisher={Cambridge university press}
}

@inproceedings{makhdoumi2013privacy,
  title={Privacy-utility tradeoff under statistical uncertainty.},
  author={Makhdoumi, Ali and Fawaz, Nadia},
  booktitle={Allerton},
  pages={1627--1634},
  year={2013}
}

@inproceedings{koh2017understanding,
  title={Understanding black-box predictions via influence functions},
  author={Koh, Pang Wei and Liang, Percy},
  booktitle={Proc. of International Conference on Machine Learning},
  year={2017}
}

@inproceedings{yeh2018representer,
  title={Representer Point Selection for Explaining Deep Neural Networks},
  author={Yeh, Chih-Kuan and Kim, Joon and Yen, Ian En-Hsu and Ravikumar, Pradeep K},
  booktitle={Proc. of Advances in Neural Information Processing Systems (NeurIPS)},
  year={2018}
}

@article{huang2017context,
  title={Context-aware generative adversarial privacy},
  author={Huang, Chong and Kairouz, Peter and Chen, Xiao and Sankar, Lalitha and Rajagopal, Ram},
  journal={Entropy},
  volume={19},
  number={12},
  pages={656},
  year={2017},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{tripathy2017privacy,
  title={Privacy-Preserving Adversarial Networks},
  author={Tripathy, Ardhendu and Wang, Ye and Ishwar, Prakash},
  journal={arXiv preprint arXiv:1712.07008},
  year={2017}
}

@book{cover2012elements,
  title={Elements of information theory},
  author={Cover, Thomas M and Thomas, Joy A},
  year={2012},
  publisher={John Wiley \& Sons}
}

@book{royden1988real,
  title={Real analysis},
  author={Royden, Halsey Lawrence and Fitzpatrick, Patrick},
  volume={32},
  year={1988},
  publisher={Macmillan New York}
}

@article{calmon2017principal,
  title={Principal Inertia Components and Applications},
  author={Calmon, Flavio P and Makhdoumi, Ali and M{\'e}dard, Muriel and Varia, Mayank and Christiansen, Mark and Duffy, Ken R},
  journal={{IEEE} Trans. Inf. Theory},
  volume={63},
  number={9},
  pages={5011--5038},
  year={2017},
  publisher={IEEE}
}

@inproceedings{calmon2015fundamental,
  title={Fundamental limits of perfect privacy},
  author={Calmon, Flavio P and Makhdoumi, Ali and M{\'e}dard, Muriel},
  booktitle={Proc. of IEEE ISIT},
  year={2015}
}

@book{tan2007introduction,
  title={Introduction to data mining},
  author={Tan, Pang-Ning and others},
  year={2007},
  publisher={Pearson Education India}
}

@article{sugiyama2010density,
  title={Density Ratio Estimation: A Comprehensive Review (Statistical Experiment and Its Related Topics)},
  author={Sugiyama, Masashi and Suzuki, Taiji and Kanamori, Takafumi},
  year={2010},
  journal={RIMS Kokyuroku},
  pages={10--31}
}

@misc{angwin2016machine,
  title={Machine bias. ProPublica, May 23, 2016},
  author={Angwin, Julia and Larson, Jeff and Mattu, Surya and Kirchner, Lauren},
  year={2016}
}

@book{sugiyama2012density,
  title={Density ratio estimation in machine learning},
  author={Sugiyama, Masashi and Suzuki, Taiji and Kanamori, Takafumi},
  year={2012},
  publisher={Cambridge University Press}
}

@inproceedings{liu2017trimmed,
  title={Trimmed Density Ratio Estimation},
  author={Liu, Song and Takeda, Akiko and Suzuki, Taiji and Fukumizu, Kenji},
  booktitle={Advances in Neural Information Processing Systems},
  pages={4518--4528},
  year={2017}
}

@article{issa2018operational,
  title={An operational approach to information leakage},
  author={Issa, Ibrahim and Wagner, Aaron B and Kamath, Sudeep},
  journal={arXiv preprint arXiv:1807.07878},
  year={2018}
}

@article{warner1965randomized,
  title={Randomized response: A survey technique for eliminating evasive answer bias},
  author={Warner, Stanley L},
  journal={Journal of the American Statistical Association},
  volume={60},
  number={309},
  pages={63--69},
  year={1965},
  publisher={Taylor \& Francis}
}

@article{sason2016f,
  title={$f$-divergence Inequalities},
  author={Sason, Igal and Verdu, Sergio},
  journal={IEEE Transactions on Information Theory},
  volume={62},
  number={11},
  pages={5973--6006},
  year={2016},
  publisher={IEEE}
}

@article{huang2018generative,
  title={Generative Adversarial Privacy},
  author={Huang, Chong and Kairouz, Peter and Chen, Xiao and Sankar, Lalitha and Rajagopal, Ram},
  journal={arXiv preprint arXiv:1807.05306},
  year={2018}
}

@book{agrawal2000privacy,
  title={Privacy-preserving data mining},
  author={Agrawal, Rakesh and Srikant, Ramakrishnan},
  volume={29},
  number={2},
  year={2000},
  publisher={ACM}
}

@article{diaz2018robustness,
  title={On the Robustness of Information-Theoretic Privacy Measures and Mechanisms},
  author={Diaz, Mario and Wang, Hao and Calmon, Flavio P and Sankar, Lalitha},
  journal={arXiv preprint arXiv:1811.06057},
  year={2018}
}

@inproceedings{verdu2015alpha,
  title={$\alpha$-mutual information},
  author={Verd{\'u}, Sergio},
  booktitle={Information Theory and Applications Workshop (ITA), 2015},
  pages={1--6},
  year={2015},
  organization={IEEE}
}

@inproceedings{du2012privacy,
  title={Privacy against statistical inference},
  author={du Pin Calmon, Fl{\'a}vio and Fawaz, Nadia},
  booktitle={Communication, Control, and Computing (Allerton), 2012 50th Annual Allerton Conference on},
  pages={1401--1408},
  year={2012},
  organization={IEEE}
}

@article{belghazi2018mine,
  title={MINE: mutual information neural estimation},
  author={Belghazi, Ishmael and Rajeswar, Sai and Baratin, Aristide and Hjelm, R Devon and Courville, Aaron},
  journal={arXiv preprint arXiv:1801.04062},
  year={2018}
}

@book{van2000empirical,
  title={Empirical Processes in M-estimation},
  author={van de Geer, Sara A and van de Geer, Sara},
  volume={6},
  year={2000},
  publisher={Cambridge university press}
}

@article{amemiya1985advanced,
  title={Asymptotic Properties of Extremum Estimators},
  author={Amemiya, Takeshi},
  journal={Advanced econometrics, Harvard university press},
  year={1985}
}

@article{tishby2000information,
  title={The information bottleneck method},
  author={Tishby, Naftali and Pereira, Fernando C and Bialek, William},
  journal={arXiv preprint physics/0004057},
  year={2000}
}

@article{hornik1989multilayer,
  title={Multilayer feedforward networks are universal approximators},
  author={Hornik, Kurt and Stinchcombe, Maxwell and White, Halbert},
  journal={Neural networks},
  volume={2},
  number={5},
  pages={359--366},
  year={1989},
  publisher={Elsevier}
}

@online{extension,
  title={Information-Theoretic Privacy Watchdog - Extended Version},
  author={Hsu, Hsiang and Asoodeh, Shahab and Calmon, Flavio P},
  url={https://github.com/HsiangHsu/ISIT-19-Extended-Version}
}

@article{liao2018tunable,
  title={A Tunable Measure for Information Leakage},
  author={Liao, Jiachun and Kosut, Oliver and Sankar, Lalitha and Calmon, Flavio P},
  journal={arXiv preprint arXiv:1806.03332},
  year={2018}
}

@book{han2013information,
  title={Information-spectrum methods in information theory},
  author={Han, Te Sun},
  year={1998},
  publisher={Tokyo, Japan: Baifukan}
}


@ARTICLE{Asoodeh_Arimoto, 
author={S. Asoodeh and M. Diaz and F. Alajaji and T. Linder}, 
journal={IEEE Trans. Inf. Theory}, 
title={Estimation Efficiency Under Privacy Constraints}, 
year={2018}, 
volume={}, 
number={}, 
pages={1-1}, 
keywords={Privacy;Random variables;Estimation;Correlation;Perturbation methods;Electronic mail;Optimization;Data privacy;privacy-utility tradeoff;guessing probability;Rényi’s entropy;minimum mean-squared error;maximal correlation;Gaussian additive privacy mechanism}, 
doi={10.1109/TIT.2018.2865558}, 
ISSN={0018-9448}, 
month={},}

@article{Csiszar67,
    author = {Csisz{\'a}r, I.},
    citeulike-article-id = {1615119},
    journal = {Studia Sci. Math. Hungar.},
    keywords = {bibtex-import},
    pages = {299--318},
    posted-at = {2007-09-03 04:57:45},
    priority = {2},
    title = {{Information-type measures of difference of probability distributions and indirect observations}},
    volume = {2},
    year = {1967}
}

@inproceedings{evfimievski2003limiting,
  title={Limiting privacy breaches in privacy preserving data mining},
  author={Evfimievski, Alexandre and Gehrke, Johannes and Srikant, Ramakrishnan},
  booktitle={Proceedings of the twenty-second ACM SIGMOD-SIGACT-SIGART symposium on Principles of database systems},
  pages={211--222},
  year={2003},
  organization={ACM}
}

@inproceedings{wang2018utility,
  title={The utility cost of robust privacy guarantees},
  author={Wang, Hao and Diaz, Mario and Calmon, Flavio P and Sankar, Lalitha},
  booktitle={Proc. of IEEE Int. Symp. Inf. Theory (ISIT)},
  year={2018}
}

@article{rassouli2017perfect,
  title={On Perfect Privacy and Maximal Correlation},
  author={Rassouli, Borzoo and Gunduz, Deniz},
  journal={arXiv preprint arXiv:1712.08500},
  year={2017}
}

@article{takbiri2018privacy,
  title={Privacy of Dependent Users Against Statistical Matching},
  author={Takbiri, Nazanin and Houmansadr, Amir and Goeckel, Dennis L and Pishro-Nik, Hossein},
  journal={arXiv preprint arXiv:1806.11108},
  year={2018}
}

@article{newey1994large,
  title={Large sample estimation and hypothesis testing},
  author={Newey, Whitney K and McFadden, Daniel},
  journal={Handbook of econometrics},
  volume={4},
  pages={2111--2245},
  year={1994},
  publisher={Elsevier}
}

@incollection{hoeffding1994probability,
  title={Probability inequalities for sums of bounded random variables},
  author={Hoeffding, Wassily},
  booktitle={The Collected Works of Wassily Hoeffding},
  pages={409--426},
  year={1994},
  publisher={Springer}
}

@book{shalev2014understanding,
  title={Understanding machine learning: From theory to algorithms},
  author={Shalev-Shwartz, Shai and Ben-David, Shai},
  year={2014},
  publisher={Cambridge university press}
}

@book{berge1997topological,
  title={Topological Spaces: including a treatment of multi-valued functions, vector spaces, and convexity},
  author={Berge, Claude},
  year={1997},
  publisher={Courier Corporation}
}

@article{mcdiarmid1989method,
  title={On the method of bounded differences},
  author={McDiarmid, Colin},
  journal={Surveys in combinatorics},
  volume={141},
  number={1},
  pages={148--188},
  year={1989},
  publisher={Norwich}
}

@inproceedings{fan2018smooth,
  title={Image Pixelization with Differential Privacy},
  author={Fan, Liyue},
  booktitle={IFIP Annual Conference on Data and Applications Security and Privacy},
  pages={148--162},
  year={2018},
  organization={Springer}
}

@inproceedings{nissim2007smooth,
  title={Smooth sensitivity and sampling in private data analysis},
  author={Nissim, Kobbi and Raskhodnikova, Sofya and Smith, Adam},
  booktitle={Proceedings of the thirty-ninth annual ACM symposium on Theory of computing},
  pages={75--84},
  year={2007},
  organization={ACM}
}

@misc{bache2013uci,
  title={{UCI} machine learning repository},
  author={Bache, Kevin and Lichman, Moshe},
  year={2013}
}

@misc{genki,
  author={},
  title = {The {MPL}ab {GENKI} {D}atabase, {GENKI-4K} {S}ubset},
  howpublished = {\url{http://mplab.ucsd.edu}},
  year={2009}
}

@inproceedings{liu2015faceattributes,
 author = {Ziwei Liu and Ping Luo and Xiaogang Wang and Xiaoou Tang},
 title = {Deep Learning Face Attributes in the Wild},
 booktitle = {Proceedings of International Conference on Computer Vision (ICCV)},
 year = {2015} 
}

@article{manning2010introduction,
  title={Introduction to information retrieval},
  author={Manning, Christopher and Raghavan, Prabhakar and Sch{\"u}tze, Hinrich},
  journal={Natural Language Engineering},
  volume={16},
  number={1},
  pages={100--103},
  year={2010},
  publisher={Cambridge university press}
}

@misc{tweet_political_bias,
  title = {Predicting Political Bias with Python},
  howpublished = {\url{https://medium.com/linalgo/predict-political-bias-using-python-b8575eedef13}},
  note = {Accessed: 2019-03-21}
}

@inproceedings{oh2017adversarial,
  title={Adversarial image perturbation for privacy protection a game theory perspective},
  author={Oh, Seong Joon and Fritz, Mario and Schiele, Bernt},
  booktitle={2017 IEEE International Conference on Computer Vision (ICCV)},
  pages={1491--1500},
  year={2017},
  organization={IEEE}
}

@inproceedings{yamada2011relative,
  title={Relative density-ratio estimation for robust distribution comparison},
  author={Yamada, Makoto and Suzuki, Taiji and Kanamori, Takafumi and Hachiya, Hirotaka and Sugiyama, Masashi},
  booktitle={Advances in neural information processing systems},
  pages={594--602},
  year={2011}
}

@inproceedings{goodfellow2014generative,
  title={Generative adversarial nets},
  author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  booktitle={Advances in neural information processing systems},
  pages={2672--2680},
  year={2014}
}

@article{polyanskiy2014lecture,
  title={Lecture notes on information theory},
  author={Polyanskiy, Yury and Wu, Yihong},
  journal={Lecture Notes for ECE563 (UIUC) and},
  volume={6},
  pages={2012--2016},
  year={2014}
}

@article{han1993approximation,
  title={Approximation theory of output statistics},
  author={Han, Te Sun and Verd{\'u}, Sergio},
  journal={IEEE Transactions on Information Theory},
  volume={39},
  number={3},
  pages={752--772},
  year={1993},
  publisher={IEEE}
}

@article{shimodaira2000improving,
  title={Improving predictive inference under covariate shift by weighting the log-likelihood function},
  author={Shimodaira, Hidetoshi},
  journal={Journal of statistical planning and inference},
  volume={90},
  number={2},
  pages={227--244},
  year={2000},
  publisher={Elsevier}
}

@article{sugiyama2007covariate,
  title={Covariate shift adaptation by importance weighted cross validation},
  author={Sugiyama, Masashi and Krauledat, Matthias and M{\~A}{\v{z}}ller, Klaus-Robert},
  journal={Journal of Machine Learning Research},
  volume={8},
  number={May},
  pages={985--1005},
  year={2007}
}

@inproceedings{smola2009relative,
  title={Relative novelty detection},
  author={Smola, Alex and Song, Le and Teo, Choon Hui},
  booktitle={Artificial Intelligence and Statistics},
  pages={536--543},
  year={2009}
}

@article{hido2011statistical,
  title={Statistical outlier detection using direct density ratio estimation},
  author={Hido, Shohei and Tsuboi, Yuta and Kashima, Hisashi and Sugiyama, Masashi and Kanamori, Takafumi},
  journal={Knowledge and information systems},
  volume={26},
  number={2},
  pages={309--336},
  year={2011},
  publisher={Springer}
}

@book{vapnik2013nature,
  title={The nature of statistical learning theory},
  author={Vapnik, Vladimir},
  year={2013},
  publisher={Springer science \& business media}
}

@article{sankar2013utility,
  title={Utility-privacy tradeoffs in databases: An information-theoretic approach},
  author={Sankar, Lalitha and Rajagopalan, S Raj and Poor, H Vincent},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={8},
  number={6},
  pages={838--852},
  year={2013},
  publisher={IEEE}
}

@article{asoodeh2019estimation,
  title={Estimation efficiency under privacy constraints},
  author={Asoodeh, Shahab and Diaz, Mario and Alajaji, Fady and Linder, Tam{\'a}s},
  journal={IEEE Transactions on Information Theory},
  volume={65},
  number={3},
  pages={1512--1534},
  year={2019},
  publisher={IEEE}
}

@article{karwa2016inference,
  title={Inference using noisy degrees: Differentially private {$beta$}-model and synthetic graphs},
  author={Karwa, Vishesh and Slavkovi{\'c}, Aleksandra and others},
  journal={The Annals of Statistics},
  volume={44},
  number={1},
  pages={87--112},
  year={2016},
  publisher={Institute of Mathematical Statistics}
}


@ARTICLE{Viswanath, 
author={Q. {Geng} and P. {Viswanath}}, 
journal={IEEE Transactions on Information Theory}, 
title={The Optimal Noise-Adding Mechanism in Differential Privacy}, 
year={2016}, 
volume={62}, 
number={2}, 
pages={925-951}, 
keywords={data privacy;query processing;statistical distributions;optimal noise-adding mechanism;statistical database;global sensitivity;optimal ϵ-differentially private mechanism;general utility-maximization framework;noise probability distributions;staircase-shaped probability density functions;discrete query output settings;simple algorithmic description;ℓ2cost functions;ℓ1cost functions;Laplacian mechanism;Privacy;Data privacy;Sensitivity;Databases;Laplace equations;Probability distribution;Context;Data privacy;randomized algorithm;Data privacy;randomized algorithm}, 
doi={10.1109/TIT.2015.2504967}, 
ISSN={0018-9448}, 
month={Feb},}


@ARTICLE{Yuri_finite, 
author={Y. {Polyanskiy} and H. V. {Poor} and S. {Verdu}}, 
journal={IEEE Transactions on Information Theory}, 
title={Channel Coding Rate in the Finite Blocklength Regime}, 
year={2010}, 
volume={56}, 
number={5}, 
pages={2307-2359}, 
keywords={channel coding;error statistics;finite blocklength regime;maximal channel coding rate;error probability;channel dispersion;complementary Gaussian cumulative distribution function;Channel coding;Error probability;Capacity planning;Channel capacity;AWGN;Codes;Distribution functions;Acoustic noise;Upper bound;Achievability;channel capacity;coding for noisy channels;converse;finite blocklength regime;Shannon theory}, 
doi={10.1109/TIT.2010.2043769}, 
ISSN={0018-9448}, 
month={May},}


@article{hockey_stick,
  author    = {N. Sharma and
               N. A. Warsi},
  title     = {Fundamental bound on the reliability of quantum information transmission},
  journal   = {CoRR},
  volume    = {abs/1302.5281},
  year      = {2013},
  url       = {http://arxiv.org/abs/1302.5281},
  archivePrefix = {arXiv},
  eprint    = {1302.5281},
  timestamp = {Mon, 13 Aug 2018 01:00:00 +0200},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}





@InProceedings{Improving_Gaussian,
  title = 	 {Improving the {G}aussian Mechanism for Differential Privacy: Analytical Calibration and Optimal Denoising},
  author = 	 {Balle, Borja and Wang, Yu-Xiang},
  booktitle = 	 {Proceedings of the 35th International Conference on Machine Learning},
  pages = 	 {394--403},
  year = 	 {2018},
  volume = 	 {80},
  month = 	 {10--15 July},
}

@article{lecam1973,
author = "LeCam, L.",
doi = "10.1214/aos/1193342380",
fjournal = "The Annals of Statistics",
journal = "Ann. Statist.",
month = "01",
number = "1",
pages = "38--53",
publisher = "The Institute of Mathematical Statistics",
title = "Convergence of Estimates Under Dimensionality Restrictions",
volume = "1",
year = "1973"
}

@ARTICLE{Gilardoni, 
author={G. L. {Gilardoni}}, 
journal={IEEE Transactions on Information Theory}, 
title={On Pinsker's and Vajda's Type Inequalities for Csiszár's$f$-Divergences}, 
year={2010}, 
volume={56}, 
number={11}, 
pages={5377-5386}, 
keywords={entropy;Vajda type inequalities;Pinsker type inequalities;Csiszár f -divergences;information divergence;total variation distance;lower bounds;Hellinger discrimination;Rényi divergences;Tsallis divergences;relative entropy;Convergence;Entropy;Convex functions;Taylor series;Probability;Loss measurement;Polynomials;Hellinger discrimination;information inequalities;Kullback–Leibler divergence;relative entropy;relative information;Rényi's information gain;variational or$L^{1}$distance}, 
doi={10.1109/TIT.2010.2068710}, 
ISSN={0018-9448}, 
month={Nov},}

@InProceedings{DP_Image,
author="Fan, L.",
editor="Kerschbaum, F.
and Paraboschi, S.",
title="Image Pixelization with Differential Privacy",
booktitle="Data and Applications Security and Privacy XXXII",
year="2018",
publisher="Springer International Publishing",
address="Cham",
pages="148--162",
abstract="Ubiquitous surveillance cameras and personal devices have given rise to the vast generation of image data. While sharing the image data can benefit various applications, including intelligent transportation systems and social science research, those images may capture sensitive individual information, such as license plates, identities, etc. Existing image privacy preservation techniques adopt deterministic obfuscation, e.g., pixelization, which can lead to re-identification with well-trained neural networks. In this study, we propose sharing pixelized images with rigorous privacy guarantees. We extend the standard differential privacy notion to image data, which protects individuals, objects, or their features. Empirical evaluation with real-world datasets demonstrates the utility and efficiency of our method; despite its simplicity, our method is shown to effectively reduce the success rate of re-identification attacks.",
isbn="978-3-319-95729-6"
}

@misc{DP_GAN,
title={Generating Differentially Private Datasets Using {GAN}s},
author={Aleksei Triastcyn and Boi Faltings},
year={2018},
url={https://openreview.net/forum?id=rJv4XWZA-},
}

@inproceedings{dwork2010boosting,
  title={Boosting and differential privacy},
  author={Dwork, Cynthia and Rothblum, Guy N and Vadhan, Salil},
  booktitle={2010 IEEE 51st Annual Symposium on Foundations of Computer Science},
  pages={51--60},
  year={2010},
  organization={IEEE}
}

@article{vzliobaite2016using,
  title={Using sensitive personal data may be necessary for avoiding discrimination in data-driven decision models},
  author={{\v{Z}}liobait{\.e}, Indr{\.e} and Custers, Bart},
  journal={Artificial Intelligence and Law},
  volume={24},
  number={2},
  pages={183--201},
  year={2016},
  publisher={Springer}
}


@ARTICLE{van_Erven, 
author={T. {van Erven} and P. {Harremos}}, 
journal={IEEE Transactions on Information Theory}, 
title={R\'enyi Divergence and Kullback-Leibler Divergence}, 
year={2014}, 
volume={60}, 
number={7}, 
pages={3797-3820}, 
keywords={algebra;entropy;minimax techniques;continuous channel inputs;minimax redundancy;channel capacity;Pythagorean inequality;Gaussian contiguity;Gaussian dichotomy;σ-algebras;continuity;convexity;Rényi entropy;Shannon entropy;Kullback-Leibler divergence;Rényi divergence;Entropy;Q measurement;Data processing;Convergence;Markov processes;Testing;\(\alpha\) -divergence;Bhattacharyya distance;information divergence;Kullback-Leibler divergence;Pythagorean inequality;Rényi divergence}, 
doi={10.1109/TIT.2014.2320500}, 
ISSN={0018-9448}, 
month={July},}

@article{abowd2016challenge,
  title={The challenge of scientific reproducibility and privacy protection for statistical agencies},
  author={Abowd, John M},
  journal={Census Scientific Advisory Committee},
  year={2016}
}

@inproceedings{ding2017collecting,
  title={Collecting telemetry data privately},
  author={Ding, Bolin and Kulkarni, Janardhan and Yekhanin, Sergey},
  booktitle={Advances in Neural Information Processing Systems},
  pages={3571--3580},
  year={2017}
}

@inproceedings{erlingsson2014rappor,
  title={Rappor: Randomized aggregatable privacy-preserving ordinal response},
  author={Erlingsson, {\'U}lfar and Pihur, Vasyl and Korolova, Aleksandra},
  booktitle={Proceedings of the 2014 ACM SIGSAC conference on computer and communications security},
  pages={1054--1067},
  year={2014},
  organization={ACM}
}

@article{chaudhuri2011differentially,
  title={Differentially private empirical risk minimization},
  author={Chaudhuri, Kamalika and Monteleoni, Claire and Sarwate, Anand D},
  journal={Journal of Machine Learning Research},
  volume={12},
  number={Mar},
  pages={1069--1109},
  year={2011}
}

@misc{Apple_Privacy,
title={Learning with privacy at scale},
author={{Differential privacy team Apple}},
year={2017},
journal={Technical report, Apple},
}


@article{liao2017hypothesis,
  title={Hypothesis testing under mutual information privacy constraints in the high privacy regime},
  author={Liao, Jiachun and Sankar, Lalitha and Tan, Vincent YF and du Pin Calmon, Flavio},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={13},
  number={4},
  pages={1058--1071},
  year={2017},
  publisher={IEEE}
}

@article{coavoux2018privacy,
  title={Privacy-preserving Neural Representations of Text},
  author={Coavoux, Maximin and Narayan, Shashi and Cohen, Shay B},
  journal={Conference on Empirical Methods in Natural Language Processing},
  year={2018}
}

@inproceedings{cuff2016differential,
  title={Differential privacy as a mutual information constraint},
  author={Cuff, Paul and Yu, Lanqing},
  booktitle={Proceedings of the 2016 ACM SIGSAC Conference on Computer and Communications Security},
  pages={43--54},
  year={2016},
  organization={ACM}
}

@inproceedings{valiant2011estimating,
  title={Estimating the unseen: an n/log (n)-sample estimator for entropy and support size, shown optimal via new CLTs},
  author={Valiant, Gregory and Valiant, Paul},
  booktitle={Proceedings of the forty-third annual ACM symposium on Theory of computing},
  pages={685--694},
  year={2011},
  organization={ACM}
}

@inproceedings{gao2017estimating,
  title={Estimating mutual information for discrete-continuous mixtures},
  author={Gao, Weihao and Kannan, Sreeram and Oh, Sewoong and Viswanath, Pramod},
  booktitle={Advances in Neural Information Processing Systems},
  pages={5986--5997},
  year={2017}
}

@article{wu2016minimax,
  title={Minimax rates of entropy estimation on large alphabets via best polynomial approximation},
  author={Wu, Yihong and Yang, Pengkun},
  journal={IEEE Transactions on Information Theory},
  volume={62},
  number={6},
  pages={3702--3720},
  year={2016},
  publisher={IEEE}
}

@article{rassouli2019optimal,
  title={Optimal utility-privacy trade-off with total variation distance as a privacy measure},
  author={Rassouli, Borzoo and Gunduz, Deniz},
  journal={IEEE Transactions on Information Forensics and Security},
  year={2019},
  publisher={IEEE}
}


@InProceedings{ZeroDP,
	author="Bun, Mark
	and Steinke, Thomas",
	title="Concentrated Differential Privacy: Simplifications, Extensions, and Lower Bounds",
	booktitle="Theory of Cryptography",
	year="2016",
	publisher="Springer Berlin Heidelberg",
	address="Berlin, Heidelberg",
	pages="635--658",
	}


@article{Concentrated_Dwork,
	author    = {C. Dwork and
	G. N. Rothblum},
	title     = {Concentrated Differential Privacy},
	volume    = {abs/1603.01887},
	year      = {2016},
	journal   = {ArXiv},
	archivePrefix = {arXiv},
	eprint    = {1603.01887},
}

@inproceedings{Barthe:2013_Beyond_DP,
	author = {Barthe, G. and Olmedo, F.},
	title = {Beyond Differential Privacy: Composition Theorems and Relational Logic for $f$-divergences Between Probabilistic Programs},
	booktitle = {ICALP},
	year = {2013},
	pages = {49--60},
} 

@inproceedings{Balle:Subsampling,
	author = {Balle, B. and Barthe, G. and Gaboardi, M.},
	title = {Privacy Amplification by Subsampling: Tight Analyses via Couplings and Divergences},
	booktitle = {Proc. 32Nd International Conference on Neural Information Processing Systems},
	series = {NIPS'18},
	year = {2018},
	location = {Montreal, Canada},
	pages = {6280--6290},
	numpages = {11},
} 

@inproceedings{RenyiDP,
	title	= {R\'enyi Differential Privacy},
	author	= {Ilya Mironov},
	year	= {2017},
	booktitle	= {Proceedings of 30th IEEE Computer Security Foundations Symposium (CSF)},
	pages	= {263-275}
}

@inproceedings{TruncatedDP,
	author = {Bun, Mark and Dwork, Cynthia and Rothblum, Guy N. and Steinke, Thomas},
	title = {Composable and Versatile Privacy via Truncated CDP},
	booktitle = {Proceedings of the 50th Annual ACM SIGACT Symposium on Theory of Computing},
	series = {STOC 2018},
	year = {2018},
	isbn = {978-1-4503-5559-9},
	location = {Los Angeles, CA, USA},
	pages = {74--86},
} 

@inproceedings{Vadhan_Composition,
	author = {Dwork, Cynthia and Rothblum, Guy N. and Vadhan, Salil},
	title = {Boosting and Differential Privacy},
	booktitle = {Proceedings of the 2010 IEEE 51st Annual Symposium on Foundations of Computer Science},
	series = {FOCS '10},
	year = {2010},
	isbn = {978-0-7695-4244-7},
	pages = {51--60},
} 

@ARTICLE{Verdu:f_divergence, 
	author={I. {Sason} and S. {Verd\'u}}, 
	journal={IEEE Transactions on Information Theory}, 
	title={$f$ -Divergence Inequalities}, 
	year={2016}, 
	volume={62}, 
	number={11}, 
	pages={5973-6006}, 
	keywords={entropy;probability;f-divergence inequalities;probability measures;arbitrary alphabets;logarithmic-convexity property;Bhattacharyya distance;relative entropy;χ2divergences;boundedness assumptions;total variation distance;reverse Pinsker inequalities;Rényi divergence;relative information spectrum;variational distance;Entropy;Information theory;Conferences;Joining processes;Q measurement;Systematics;Integral equations;Relative entropy;total variation distance;f-divergence;Rényi divergence;Pinsker’s inequality;relative information}, 
	doi={10.1109/TIT.2016.2603151}, 
	ISSN={0018-9448}, 
	month={Nov},}

@article{Balle2019HypothesisTI,
	title={Hypothesis Testing Interpretations and {R\'enyi} Differential Privacy},
	author={Borja Balle and Gilles Barthe and Marco Gaboardi and Justin Hsu and Tetsuya Sato},
	journal={ArXiv},
	year={2019},
	volume={abs/1905.09982}
}

%%inproceedings{Balle2018Subsampling,
%	title={Privacy Amplification by Subsampling: Tight Analyses via Couplings and Divergences},
%	author={Borja Balle and Gilles Barthe and Marco Gaboardi},
%	booktitle={NeurIPS},
%	year={2018}
%}

@article{Balle2019mixing,
	title={Privacy Amplification by Mixing and Diffusion Mechanisms},
	author={Borja Balle and Gilles Barthe and Marco Gaboardi and Joseph Geumlek},
	journal={ArXiv},
	year={2019},
	volume={abs/1905.12264}
}


@InProceedings{Poisson_Subsample_RDP,
	title = 	 {Poission Subsampled R\'enyi Differential Privacy},
	author = 	 {Zhu, Yuqing and Wang, Yu-Xiang},
	booktitle = 	 {Proceedings of the 36th International Conference on Machine Learning},
	pages = 	 {7634--7642},
	year = 	 {2019},
	editor = 	 {Chaudhuri, Kamalika and Salakhutdinov, Ruslan},
	volume = 	 {97},
	month = 	 {09--15 Jun},
}

@inproceedings{Balle_AnalyticMomentAccountant,
	title={Subsampled {R\'enyi} Differential Privacy and Analytical Moments Accountant},
	author={Yu-Xiang Wang and Borja Balle and Shiva Prasad Kasiviswanathan},
	booktitle={AISTATS},
	year={2018}
}

@article{Csiszar_Sheilds,
	author = {Csisz\'{a}r, Imre and Shields, Paul C.},
	title = {Information Theory and Statistics: A Tutorial},
	journal = {Commun. Inf. Theory},
	issue_date = {December 2004},
	volume = {1},
	number = {4},
	month = dec,
	year = {2004},
	issn = {1567-2190},
	pages = {417--528},
	numpages = {112},
	url = {http://dx.doi.org/10.1561/0100000004},
	doi = {10.1561/0100000004},
	acmid = {1166380},
	publisher = {Now Publishers Inc.},
	address = {Hanover, MA, USA},
} 

@INPROCEEDINGS{Issa_Operational, 
	author={I. {Issa} and A. B. {Wagner}}, 
	booktitle={2017 IEEE International Symposium on Information Theory (ISIT)}, 
	title={Operational definitions for some common information leakage metrics}, 
	year={2017}, 
	volume={}, 
	number={}, 
	pages={769-773}, 
	keywords={data privacy;information theory;statistical distributions;telecommunication network reliability;telecommunication security;operational definitions;common information leakage metrics;maximal leakage;randomized function;guessing framework;Shannon capacity;maximal correlation;local differential privacy;correct guessing probability;maximum information rate;valid leakage measure;Correlation;Privacy;Measurement;Mutual information;Random variables;Reliability}, 
	doi={10.1109/ISIT.2017.8006632}, 
	ISSN={2157-8117}, 
	month={June},}

@INPROCEEDINGS{Issa_Leakage, 
	author={I. {Issa} and S. {Kamath} and A. B. {Wagner}}, 
	booktitle={2016 Annual Conference on Information Science and Systems (CISS)}, 
	title={An operational measure of information leakage}, 
	year={2016}, 
	volume={}, 
	number={}, 
	pages={234-239}, 
	keywords={data privacy;random processes;information leakage;operational measure;discrete random variables;maximal leakage;randomized function;Sibson mutual information;order infinity;data processing inequality;true function value;Measurement;Privacy;Security;Random variables;Mutual information;Semantics;Information science;Leakage;Privacy;Sibson mutual information;Inference},
	doi={10.1109/CISS.2016.7460507}, 
	ISSN={}, 
	month={March},}





@ARTICLE{Csiszar, 
	author={I. {Csiszar}}, 
	journal={IEEE Transactions on Information Theory}, 
	title={Generalized cutoff rates and Renyi's information measures}, 
	year={1995}, 
	volume={41}, 
	number={1}, 
	pages={26-34}, 
	keywords={channel coding;channel capacity;encoding;block codes;entropy;generalized cutoff rates;Renyi's information measures;entropy;divergence;block coding;hypothesis testing;/spl beta/-cutoff rates;mutual information;channel capacity;channel coding;Entropy;Testing;Block codes;Channel capacity;Q measurement;Mutual information;Channel coding;Information theory;Terminology;Books}, 
	doi={10.1109/18.370121}, 
	ISSN={0018-9448}, 
	month={Jan},}


@INPROCEEDINGS{Verdu_alphaMI, 
	author={S. {Verd\'u}}, 
	booktitle={2015 Information Theory and Applications Workshop (ITA)}, 
	title={$\alpha$-mutual information}, 
	year={2015}, 
	volume={}, 
	number={}, 
	pages={1-6}, 
	doi={10.1109/ITA.2015.7308959}, 
	ISSN={}, 
	month={Feb},}


@ARTICLE{Yury_Dissipation, 
	author={Y. {Polyanskiy} and Y. {Wu}}, 
	journal={IEEE Transactions on Information Theory}, 
	title={Dissipation of Information in Channels With Input Constraints}, 
	year={2016}, 
	volume={62}, 
	number={1}, 
	pages={35-55}, 
	keywords={error statistics;Gaussian channels;information theory;channel information;input constraints;information theory;data processing inequality;input divergence;Dobrushin coefficient;input cost constraint;contraction coefficient;Dobrushin curve;additive noise channels;stochastic control;Gibbs measurement;noisy circuits;power constrained relays;Gaussian channels;end-to-end mutual information;maximal squared correlation decay;exponential decay;discrete channels;signal-to-noise ratio;SNR;bit error probability;TV;Markov processes;Relays;Kernel;Correlation;Signal to noise ratio;Strong data processing inequalities;Dobrushin’s contraction;stochastic control;Gibbs measure;noisy circuits;broadcasting on trees;Strong data processing inequalities;Dobrushin’s contraction;stochastic control;Gibbs measure;noisy circuits;broadcasting on trees}, 
	doi={10.1109/TIT.2015.2482978}, 
	ISSN={0018-9448}, 
	month={Jan},}

@article{ahlswede1976,
	author = "Ahlswede, Rudolf and G\'acs, Peter",
	doi = "10.1214/aop/1176995937",
	fjournal = "The Annals of Probability",
	journal = "Ann. Probab.",
	month = "12",
	number = "6",
	pages = "925--939",
	publisher = "The Institute of Mathematical Statistics",
	title = "Spreading of Sets in Product Spaces and Hypercontraction of the Markov Operator",
	volume = "4",
	year = "1976"
}


@article{Vitaly_AmplificationB,
	title={Privacy Amplification by Iteration},
	author={Vitaly Feldman and Ilya Mironov and Kunal Talwar and Abhradeep Thakurta},
	journal={2018 IEEE 59th Annual Symposium on Foundations of Computer Science (FOCS)},
	year={2018},
	pages={521-532}
}

@article{Feldman2018PrivacyAB,
	title={Privacy Amplification by Iteration},
	author={Vitaly Feldman and Ilya Mironov and Kunal Talwar and Abhradeep Thakurta},
	journal={2018 IEEE 59th Annual Symposium on Foundations of Computer Science (FOCS)},
	year={2018},
	pages={521-532}
}


@ARTICLE{Raginsky_SDPI, 
	author={M. {Raginsky}}, 
	journal={IEEE Transactions on Information Theory}, 
	title={Strong Data Processing Inequalities and$\Phi $-Sobolev Inequalities for Discrete Channels}, 
	year={2016}, 
	volume={62}, 
	number={6}, 
	pages={3355-3389}, 
	ISSN={0018-9448}, 
	month={June},}
	
	
	@book{cohen1998comparisons,
  title={Comparisons of Stochastic Matrices, with Applications in Information Theory, Statistics, Economics, and Population Sciences},
  author={Cohen, J.E. and Kemperman, J.H.B. and Zb{\u{a}}ganu, G.},
  isbn={9780817640828},
  lccn={98016659},
  url={https://books.google.com/books?id=oArvAAAAMAAJ},
  year={1998},
  publisher={Birkh{\"a}user}
}

@inproceedings{Abadi_MomentAccountant,
 author = {Abadi, Martin and Chu, Andy and Goodfellow, Ian and McMahan, H. Brendan and Mironov, Ilya and Talwar, Kunal and Zhang, Li},
 title = {Deep Learning with Differential Privacy},
 booktitle = {Proc. of CCS},
 year = {2016},
 isbn = {978-1-4503-4139-4},
 location = {Vienna, Austria},
 pages = {308--318},
} 

@inproceedings{Bun:tCDP,
 author = {Bun, Mark and Dwork, Cynthia and Rothblum, Guy N. and Steinke, Thomas},
 title = {Composable and Versatile Privacy via Truncated CDP},
 booktitle = {Proceedings of the 50th Annual ACM SIGACT Symposium on Theory of Computing},
 series = {STOC 2018},
 year = {2018},
 isbn = {978-1-4503-5559-9},
 location = {Los Angeles, CA, USA},
 pages = {74--86},
 numpages = {13},
 url = {http://doi.acm.org/10.1145/3188745.3188946},
 doi = {10.1145/3188745.3188946},
 acmid = {3188946},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {algorithmic stability, differential privacy, subsampling},
} 

@ARTICLE{Harremoes_JOintRange,
author={P. {Harremo\"es} and I. {Vajda}},
journal={IEEE Transactions on Information Theory},
title={On Pairs of $f$-Divergences and Their Joint Range},
year={2011},
volume={57},
number={6},
pages={3230-3235},
keywords={convex programming;information theory;statistical testing;convex hull;convex analysis;joint range;Joints;Atmospheric measurements;Particle measurements;Convex functions;Loss measurement;Density measurement;Testing;Convexity;$f$-divergence;joint range},
doi={10.1109/TIT.2011.2137353},
ISSN={},
month={June},}


@book{Choquet,
  title={Lectures on Choquet's Theorem},
  author={Phelps, R.R.},
  isbn={9783540487197},
  series={Lecture Notes in Mathematics},
  url={https://books.google.com/books?id=4UdsCQAAQBAJ},
  year={2003},
  publisher={Springer Berlin Heidelberg}
}


@inproceedings{RDP_SemiSupervised,
title	= {Semi-supervised Knowledge Transfer for Deep Learning from Private Training Data},
author	= {Nicolas Papernot and Martín Abadi and Úlfar Erlingsson and Ian Goodfellow and Kunal Talwar},
year	= {2017},
booktitle	= {Proceedings of the International Conference on Learning Representations}
}

@incollection{RDP2_PosteriorSampling,
title = {R\'enyi Differential Privacy Mechanisms for Posterior Sampling},
author = {Geumlek, Joseph and Song, Shuang and Chaudhuri, Kamalika},
booktitle = {Advances in Neural Information Processing Systems 30},
pages = {5289--5298},
year = {2017},
}

@inproceedings{Bassily1,
 author = {Bassily, Raef and Smith, Adam and Thakurta, Abhradeep},
 title = {Private Empirical Risk Minimization: Efficient Algorithms and Tight Error Bounds},
 booktitle = {Proceedings of FOCS},
 year = {2014},
 isbn = {978-1-4799-6517-5},
 pages = {464--473},
 numpages = {10},
 url = {https://doi.org/10.1109/FOCS.2014.56},
 doi = {10.1109/FOCS.2014.56},
 acmid = {2707412},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
}

@conference {BAssily2,
	title = {Private Empirical Risk Minimization, Revisited},
	booktitle = {ICML 2014 Workshop on Learning, Security and Privacy},
	year = {2014},
	month = {25 Jun},
	address = {Beijing, China},
	url = {http://arxiv.org/abs/1405.7085},
	author = {Raef Bassily and Smith, Adam and Abhradeep Thakurta}
}


@article{Wasserman,
author = {Larry Wasserman and Shuheng Zhou},
title = {A Statistical Framework for Differential Privacy},
journal = {Journal of the American Statistical Association},
volume = {105},
number = {489},
pages = {375-389},
year  = {2010},
publisher = {Taylor & Francis},
doi = {10.1198/jasa.2009.tm08651},}

@inproceedings{Shokri:DeepLearning,
 author = {Shokri, Reza and Shmatikov, Vitaly},
 title = {Privacy-Preserving Deep Learning},
 booktitle = {Proc. of CCS},
 year = {2015},
 isbn = {978-1-4503-3832-5},
 location = {Denver, Colorado, USA},
 pages = {1310--1321},
}

@ARTICLE{Kairouz_Composition,
author={P. {Kairouz} and S. {Oh} and P. {Viswanath}},
journal={IEEE Transactions on Information Theory},
title={The Composition Theorem for Differential Privacy},
year={2017},
volume={63},
number={6},
pages={4037-4049},
keywords={data privacy;composition theorem;privatization mechanisms;differential privacy;data processing inequality;Databases;Privacy;Data privacy;Testing;Data processing;Privatization;Electronic mail;Differential privacy;hypothesis testing},
doi={10.1109/TIT.2017.2685505},
ISSN={},
month={June},}



@article{Ali1966AGC,
  title={A General Class of Coefficients of Divergence of One Distribution from Another},
  author={Sami M. Ali and S. D. Silvey},
  journal = {Journal of Royal Statistics},
  volume = {28},
  pages = {131--142},
  year={1966}
}







%%InProceedings{Balle_AnalyticMomentAccountant,
%   title = 	 {Subsampled Renyi Differential Privacy and Analytical Moments Accountant},
%   author = 	 {Wang, Yu-Xiang and Balle, Borja and Kasiviswanathan, Shiva Prasad},
%   booktitle = 	 {Proceedings of Machine Learning Research},
%   pages = 	 {1226--1235},
%   year = 	 {2019},
%   editor = 	 {Chaudhuri, Kamalika and Sugiyama, Masashi},
%   volume = 	 {89},
%   series = 	 {Proc. of Machine Learning Research},
%   address = 	 {},
%   month = 	 {16--18 Apr},
% }

@misc{bhowmick2018protection,
    title={Protection Against Reconstruction and Its Applications in Private Federated Learning},
    author={Abhishek Bhowmick and John Duchi and Julien Freudiger and Gaurav Kapoor and Ryan Rogers},
    year={2018},
    eprint={1812.00984},
    archivePrefix={arXiv},
    primaryClass={stat.ML}
}

@inproceedings{Dwork_Calibration,
 author = {Dwork, Cynthia and McSherry, Frank and Nissim, Kobbi and Smith, Adam},
 title = {Calibrating Noise to Sensitivity in Private Data Analysis},
 booktitle = {Proceedings of the Third Conference on Theory of Cryptography},
 series = {TCC'06},
 year = {2006},
 location = {New York, NY},
 pages = {265--284},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
}



@article{Ours_LongVersion,
author = {S. Asoodeh and J. Liao and F. P. Calmon and Oliver Kosut and L. Sankar },
title = {A Better Bound Gives A Hundred Rounds:Enhanced Privacy Guarantees via $f$-Divergence},
url = {https://scholar.harvard.edu/files/shahab/files/isit2020_dp.pdf},
}


@book{Pinsker1964InformationAI,
  title={Information and information stability of random variables and processes},
  author={Mark A. Pinsker},
  year={1964},
  publisher= {Holden-Day},
}

@inproceedings{SGD_Exponential_VS_Gaussian,
 author = {Wu, Xi and Li, Fengan and Kumar, Arun and Chaudhuri, Kamalika and Jha, Somesh and Naughton, Jeffrey},
 title = {Bolt-on Differential Privacy for Scalable Stochastic Gradient Descent-based Analytics},
 booktitle = {SIGMOD},
 year = {2017},
 pages = {1307--1322},
 numpages = {16},
 keywords = {differential privacy, optimization, scalable data analytics, stochastic gradient descent},
} 

@article{McMahan_Privacy,
  author    = {H. Brendan McMahan and
               Galen Andrew and \'Ulfar Erlingsson and Steve Chien and
Ilya Mironov and Peter Kairouz},
  title     = {A General Approach to Adding Differential Privacy to Iterative Training
               Procedures},
  year      = {2018},
  url       = {http://arxiv.org/abs/1812.06210},
}

@article{TensorFlowPrivacy,
  author    = {{Google}},
  title     = {TensorFlow Privacy},
  year      = {2018},
  url       = {https://github.com/tensorflow/privacy},
}


